ChartGemma: Visual Instruction-tuning for Chart Reasoning in the Wild

Given the ubiquity of charts as a data analysis, visualization, and decision-making tool across industries and sciences, there has been a growing interest in developing pre-trained foundation models as well as general purpose instruction-tuned models for chart understanding and reasoning. However, existing methods suffer crucial drawbacks across two critical axes affecting the performance of chart representation models: they are trained on data generated from underlying data tables of the charts, ignoring the visual trends and patterns in chart images, and use weakly aligned vision-language backbone models for domain-specific training, limiting their generalizability when encountering charts in the wild. We address these important drawbacks and introduce ChartGemma, a novel chart understanding and reasoning model developed over PaliGemma. Rather than relying on underlying data tables, ChartGemma is trained on instruction-tuning data generated directly from chart images, thus capturing both high-level trends and low-level visual information from a diverse set of charts. Our simple approach achieves state-of-the-art results across $5$ benchmarks spanning chart summarization, question answering, and fact-checking, and our elaborate qualitative studies on real-world charts show that ChartGemma generates more realistic and factually correct summaries compared to its contemporaries. We release the code, model checkpoints, dataset, and demos at https://github.com/vis-nlp/ChartGemma.

==> Dataset.tex <==


 
 
  
  
  
                                             
  
  
 






  
  

  




  
  
  

To build a large and diverse corpus 
with various styles, topics, and storage formats, we crawled charts from various online sources. Additionally, we utilized publicly available chart datasets suitable for pretraining. The collected charts can be categorized into two types: charts with underlying data tables and charts without data tables.



\vspace{-1mm}
\subsection{Charts with Data Tables} \label{subsec:charts-data}


Charts with an underlying data table are collected in three ways: \Ni utilize existing datasets, \Nii extract SVG charts, and \Niii data augmentation.

\textbf{$\bullet$ Utilize Existing Datasets} Our goal was to train the model based on real-world data, thus, we did not consider the ones that are generated from synthetic data~\cite{dvqa, figureqa}. 
In particular, we used the following five chart datasets for which the underlying data tables were available: 
\Ni Statista ({\href{https://www.statista.com}{statista.com}})~\cite{chart-to-text-acl}, \Nii Our World In Data or OWID {(\href{https://ourworldindata.org}{ourworldindata.org})} \cite{masry-etal-2022-chartqa}, \Niii Organisation for Economic Co-operation and Development or OECD {(\href{https://www.oecd.org}{oecd.org})} \cite{masry-etal-2022-chartqa}, \Niv PlotQA~\cite{plotqa}, and \Nv a subset of the ChartInfo~\cite{chartinfo}  dataset that provides bounding box annotations for data encoding marks (e.g., bars in a bar chart). 

\textbf{$\bullet$ Extract SVG Charts:} We extracted charts in SVG format from the Chartblocks and Plotly datasets of the Beagle corpus \cite{battle2018beagle}. These charts do not come with data tables, but the data can be extracted accurately from the SVG elements. 
The steps for preparing these charts are: (1) identify axis labels and legends using specific class names of HTML attribute, (2) extract bounding boxes of chart elements (e.g., bars, line) using SVG attribute properties (e.g., \texttt{size} and \texttt{location} of \texttt{<rect>}), (3) construct the underlying data table by iterating through each of the \texttt{<g>} elements  to find data values of each data attribute.
When data labels are absent, we utilize the scale information based on the axis labels and tick marks %
of the chart and the bounding box information of data encoding marks to recover the data values.

\textbf{$\bullet$ Data Augmentation} We further augmented the corpus by creating charts from publicly available data tables. We used the {The Web Data Commons 
 (WDC)~\cite{webdatacommons}, which used Common Crawl\footnote{https://commoncrawl.org/} to collect a large amount of structured data. 
The charts are created in the following steps: 

\begin{enumerate} [wide, label=(\roman*),labelwidth=!, itemindent=!, labelindent=0pt]
\vspace{-2mm}
    \item \textit{Data pre-processing:} Since many tables in WDC contain more than three columns, we decomposed so that tables are suitable for creating desired chart types (e.g., bars, lines, and pie charts). In particular, we automatically analyze the data type of each column (e.g, numeric vs. categorical) and then randomly choose one column with numeric data values and one/two column(s) with categorical data. We also limit the maximum number of rows of the table to 8 so that the corresponding chart can fit within reasonable screen space. 
\vspace{-2mm}

    \item \textit{Chart generation}: To generate visually diverse charts, we used the D3 \cite{d3} library that provides great flexibility in terms of creating diverse visualization styles. We also employed Vega-Lite \cite{vegalite} which creates charts based on declarative JSON syntax. We used simple heuristics for determining chart types from the data table~\cite{mackinlay2007show}. We created four types of charts: (1) vertical simple bar charts with one numeric data column, (2) vertical grouped bar charts, (3) pie charts, and (4) line charts (both single series and multi-series).
\vspace{-2mm}
    \item  \textit{Visual diversification}: To create visually diverse charts resembling real-world variations, we  manipulated the following visual style properties: (1) \textbf{Colors and shapes}: Color schemes from ColorBrewer\footnote{https://colorbrewer2.org/} and Tableau\footnote{tableau.com} were chosen for categorical data attributes. We also varied shape properties such as bar thickness, line types (e.g., continuous vs dotted), and legend shape types (e.g., rect, circle). (2) \textbf{Position and distance}: We also varied bar positions and distances with respect to axis labels. (3) \textbf{Guides}: Charts may contain additional guides such as grids, so we generate charts with and without grids to diversify styles. 
\end{enumerate}

\Cref{fig:d3-samples} depicts a visually diverse set of charts created using this augmentation process. In total, we created a total of 189,839 charts (\Cref{tab:datasets}).



\subsection{Charts without Data Tables}
Many online charts are available only as images, without corresponding data tables.
However,  they can still be valuable for large-scale pretraining as we can extract chart elements and rich textual contents (e.g., titles, surrounding texts, captions) using object detection and optical character recognition (OCR) techniques. We collected image chart datasets such as LineCap \cite{mahinpei2022linecap} and Neural Caption Generation \cite{Andrea-carenini} 
since they provide high-quality summaries. We also used the Pew dataset from \cite{chart-to-text-acl} and further augmented it by an crawling additional 1K charts.
Finally, we used the ExcelChart400K dataset \cite{ChartOCR} which only provides bounding boxes without underlying data tables. We also considered other existing image chart datasets such as Vis30K \cite{chen2021vis30k} and VisImage \cite{deng2020visimages}, 
but they are not suitable as they usually have poor resolution and lack meaningful textual content (e.g., titles). 








}



\subsection{Augmentation by Knowledge Distillation for Chart-to-text Generation Tasks}
\label{subsec:knowledge_distillation}


Chart-related downstream tasks such as chart summarization \cite{chart-to-text-acl} and open-ended question answering~\cite{open-CQA} require generating informative and relevant texts. However, 
for most of the charts in the pretraining corpus, there are either no associated summaries or the summaries that are collected opportunistically such as the Statista dataset \cite{chart-to-text-acl} lack quality (e.g., too short and not very informative). {Training on such substandard ``ground-truth'' summaries can negatively affect the overall model performance as shown in text summarization \cite{kryscinski-etal-2019-neural,clark-etal-2021-thats}. Indeed, \citet{goyal2022news} and \citet{yixin-acl23} have recently shown that human raters prefer summaries generated by LLMs, especially the ones that are instruction-tuned such as InstructGPT \cite{instructgpt}, compared to the reference summaries in various text summarization datasets. Consequently, the instruction-tuned LLMs have been successfully used as a 
annotator in several recent studies \cite{Ding-acl-23,qin2023chatgpt}.



Inspired by these findings, we leveraged
InstructGPT to generate coherent and relevant text. 
Specifically, we prompted \texttt{text-davinci-003} by providing the underlying data table as input and one exemplar (i.e., 1-shot in-context learning). %
Since generating summaries for 
thousands of charts by calling OpenAI API is quite costly, we devised a knowledge distillation approach. We first used \texttt{text-davinci-003} to create a small dataset of 3700 summaries for different chart types. Next, we finetuned Flan-T5 XL \cite{chung2022scaling} on this dataset. Finally, we utilized the finetuned Flan-T5 model to generate summaries for charts that do not have an associated summary. More details about this approach can be found in \Cref{app:knowledge-distillation}. %
 
 
 
 








\subsection{Datasets Analysis}

Our chart pretraining corpus has over 611K charts covering a diverse range of bar charts, line charts, and pie charts (\Cref{tab:datasets}). Data tables of \textit{Simple} charts have two columns (simple bar charts or single-series line charts), whereas \textit{Complex} charts involve at least three columns (e.g., stacked or group bar charts, line charts with multiple lines). The first two chart groups in \Cref{tab:datasets} come with an underlying data table which cover over 80\% of the corpus.
The bottom group contains five datasets which only provide charts in image format without a data table\footnote{The ExcelChart400K dataset only provides bounding box annotations of chart elements and we used this dataset for data value estimation task during pretraining.}
and cover about 20\% of the corpus. 
Bar charts make up the majority portion (58.51\%), followed by line charts (32.94\%) and pie charts (9.39\%). About 60\% of the charts have multiple columns in their data tables, while 40\% of the charts have only two columns.\footnote{
Since we do not have access to the chart types of Pew dataset, 
we manually tagged random  200 samples from each of these datasets 
to estimate the chart type distribution.} 
The corpus also covers a diverse range of topics including technology, economy, politics, health, and society. To ensure a fair evaluation, we excluded charts found in the validation and test sets of the downstream tasks from our pretraining corpus. Details about the linguistics of the corpus textual elements can be found in \Cref{app:dataset-analysis}. 












 
  
  
  
                                             
  
  




  
  

 
 
 
 
  
  
  
  
  


  




  
  
 
 
 
 











 
  
  
  
                                             
  
  
 






  

  




  
  
  

 
  
  
  
                                             
  
  




  
  






==> Downstream.tex <==
\subsection{Downstream Tasks}


In addition to zero-shot evaluation, we also adapt \model\ by finetuning it on a downstream task. We consider four downstream tasks: \emph{(1) Factoid Chart Question Answering:} we use ChartQA \cite{masry-etal-2022-chartqa}, which is a benchmark consisting of factoid question-answer pairs for charts with a particular focus on visual and logical reasoning questions; \emph{(2) Complex Chart Question Answering:} we consider OpenCQA \cite{open-CQA}, another QA benchmark in which answers are explanatory descriptions; \emph{(3) Chart Summarization:}  we use Chart-to-Text \cite{chart-to-text-acl}, a large-scale benchmark for chart summarization; \emph{(4) Chart-to-Table:} we use ChartQA for both finetuning and evaluation. Moreover,  we evaluate the pretrained model in a zero-shot setup on the WebCharts dataset \cite{Choi2019VisualizingFT}, a collection of 300 charts obtained from the web. %


\subsection{Experiments Setup}
To minimize the computational resource requirements, we initialize our model from the base Donut weights \cite{kim2022ocr}. Our pretraining process consists of two stages. In the first stage, we set the input image resolution to 512x512 and pretrain for 300K steps. In the second stage, we increase the input image resolution to 960x960 and pretrain for an additional 100K steps. \Cref{tab:finetuning-details} shows the hyperparameters we used in pretraining and finetuning our model on each downstream task. All our experiments were carried out using one 4-A100 (40GB), one 4-A100 (80GB), and one 4-V100 (32 GB) GPU machines.  


==> Evaluation.tex <==
\begin{table*}[t]
 \setlength\extrarowheight{2pt}
 \centering
 
 
 
 \scalebox{0.73}{\begin{tabular}{l|c|cccccccc}
  
  \toprule
  
  \multirow{3}{*}{} & \multirow{3}{*}{} & \multicolumn{3}{c}{ChartQA} & 
  OpenCQA & \multicolumn{2}{c}{Chart-to-Text} & \multicolumn{2}{c}{Chart-to-Table}   \\ 
  \multirow{3}{*}{} & \multirow{3}{*}{} & \multicolumn{3}{c}{\small ($RA$)} & \small ($BLEU$) & \multicolumn{2}{c}{\small ($BLEU$)} & \multicolumn{2}{c}{\small ($RNSS$ | $RMS_{F1}$)} \\
  \cmidrule(lr){3-5} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
  
   Model & \#Params & aug. & human & avg. & OpenCQA & Pew & Statista & ChartQA & WebCharts \\
                                             
  
  \midrule

  VisionTaPas \cite{masry-etal-2022-chartqa} & - & 61.44 & 29.60 & 45.52 
  &- & - & - & - & - \\ 

  T5 \cite{masry-etal-2022-chartqa} & 222M & 56.96 & 25.12 & 41.04 
  & 9.28 & 10.49 & 35.29 & - & -  \\

  VL-T5 \cite{masry-etal-2022-chartqa} & - & 56.88 & 26.24 & 41.56 & 
  14.73 & - & - & - & -  \\ 

  Pix2Struct \cite{lee2022pix2struct} & 282M & 81.6 & 30.5 & 56.0 
  & - & 10.3 & 38.0 & - & - \\

  MatCha \cite{liu2022matcha} & 282M & \textbf{90.2} & 38.2 & 64.2
  & - & 12.2 & \textbf{39.4} & 85.21 | 83.49 & 44.37 | 17.94 \\ \midrule

  \model\ & 201M & 88.56 & \textbf{43.92} & \textbf{66.24} 
  & \textbf{14.88} & \textbf{12.48} & 38.21 & \textbf{94.01} | \textbf{91.10} & \textbf{60.73} | \textbf{43.21} \\ \bottomrule
  
  
 
 \end{tabular}}
 \vspace{-3mm}
 \caption{\small {Evaluation results on four public benchmarks: ChartQA, Chart-to-Text, OpenCQA, and Chart-to-Table. All the results are calculated after finetuning \model\ pretrained checkpoint except for WebCharts (zero-shot). %
 }
 \vspace{-3mm}
 }
 \label{tab:results}
\end{table*}
 \vspace{-2mm}
\section{Evaluation}
 \vspace{-1mm}
\subsection{Baselines \& Evaluation Metrics} \label{subsec:baselines}
We compare our model against five baselines: (1) \emph{T5} \cite{Raffel2020t5}, a unified seq2seq Transformer model that achieved state-of-the-art (SoTA) results on various text-to-text tasks, including question answering and summarization; (2) \emph{VL-T5} \cite{vlt5}, a T5-based model that unifies Vision-Language (VL) tasks as text generation conditioned on multimodal inputs and achieved SoTA results on OpenCQA \cite{open-CQA}; (3) \emph{VisionTapas} \cite{masry-etal-2022-chartqa}, an extension of TaPas \cite{tapas}, a SoTA table encoder, adapted for QA over charts; (4) \emph{Pix2Struct} \cite{lee2022pix2struct}, a pretrained image-to-text model for visual language understanding
and achieved SoTA results on document understanding tasks; and (5) \emph{MatCha} \cite{liu2022matcha}, an adapted version of Pix2Struct for charts that is further pretrained on math reasoning and chart data extraction tasks, achieving SoTA results on Chart-to-Text \cite{chart-to-text-acl} and ChartQA \cite{masry-etal-2022-chartqa}.


To evaluate our approach, we follow previous works \cite{lee2022pix2struct, chart-to-text-acl, masry-etal-2022-chartqa, open-CQA, liu2022matcha} and utilize Relaxed Accuracy (RA) for ChartQA and BLEU \cite{post-2018-call} for text-generation tasks (Chart-to-Text and OpenCQA). However, the BLEU score has limitations as it primarily focuses on n-gram matching between the generated and reference texts, overlooking important factors such as semantic similarity, informativeness, and factual correctness \cite{goyal2022news}.
 Therefore, we conduct a human evaluation and ChatGPT-driven study to assess and compare these crucial aspects in the outputs of different models (\Cref{subsec:summary_eval}). Finally, we  use Relative Number Set Similarity (RNSS) \cite{masry-etal-2022-chartqa} and Relative Mapping Similarity (RMS) \cite{liu2022deplot} metrics to evaluate the Chart-to-Table task. 








  
  
  
                                            
  

 

\subsection{Main Results}


As shown in \Cref{tab:results}, \model\ outperforms previous state-of-the-art models, MatCha and VL-T5, on the ChartQA and Chart-to-Text (Pew) datasets, although it shows slightly lower performance on Chart-to-Text (Statista). 
The performance gap is more prominent on the challenging human-written questions in the ChartQA benchmark~\cite{masry-etal-2022-chartqa}, where our model's pretraining objectives tailored to visual and numerical reasoning give it a significant advantage.
\model\ also achieved a higher BLUE score compared to the SoTA VL-T5 model on OpenCQA benchmark, which demonstrates our model's capability in generating explanatory answers for questions about charts. Finally, \model\ surpasses MatCha's performance on two datasets, demonstrating its generalizability across diverse visual styles, even in a zero-shot setup on unseen charts (WebCharts). 
Overall, these results establish \model\ as the SoTA model for chart comprehension and reasoning tasks.



To further assess the impact of our different pretraining objectives on our model's performance, we conducted ablation studies. We observe that removing various pertaining objectives led to a slight decrease in performance (\Cref{tab:ablations}). The decrease in performance is particularly noticeable when the Numerical Reasoning pretaining task is removed, highlighting the importance of this task in imbuing numerical abilities into our model.  More details of this experiment can be found in \Cref{app:ablation}.





  
  
  
                                            
  

 

















\begin{table}[t]
 \setlength\extrarowheight{2pt}
 \centering
 
 
 \scalebox{0.73}{\begin{tabular}{l|ccc}
  
  \toprule
   \textbf{Summary} & \textbf{Human} & \textbf{ChatGPT} & \textbf{p-value}\\ \midrule
   \model\ ZeroShot & \textbf{3.97} & \textbf{3.18} & 1.70e-10\\ 
   \model\ Finetuned & 2.86 & 2.37 & 2.32e-8 \\ 
   MatCha \cite{liu2022matcha} & 2.50 & 2.18 & 0.0020\\ 
   Gold \cite{chart-to-text-acl} & 3.19 & 2.73 & 2.13e-6 \\
   \bottomrule

 \end{tabular}}
 \vspace{-3mm}
 \caption{
  \small{Average Informativeness scores from Human and ChatGPT-based evaluation. 
  }
  \vspace{-4mm}
 }
 
 \label{tab:informativeness}
\end{table}
\vspace{-1mm}
\subsection{Human and ChatGPT Evaluation}
\label{subsec:summary_eval}

As discussed in \Cref{subsec:baselines}, reference-based metrics like BLEU 
have relatively low correlations with human judgments \cite{belz-reiter-2006-comparing,tan-etal-2015-awkward,liu2023geval}, and generated texts with very high such scores can be of a very poor quality \cite{smith-etal-2016-climbing}. %
Therefore, we decided to conduct a human evaluation to measure the quality of summaries generated by different models. We focus on following criteria in the chart summarization task:\emph{(1) Informativeness}; \emph{(2) Factual Correctness}; and\emph{(3) Semantic Levels that characterize the content of the summary}. More details about the criteria can be found in \Cref{app:human-chatgpt-eval}.


We randomly picked 150 sample charts from Chart2text Statista test split and asked  3 human annotators to rate four summaries for each chart based on \textit{informativeness} out of 1 to 5.  The order of exposure of summaries to the annotator was randomized to avoid any potential bias. Summaries for each chart were rated by one annotator except for the first 100 charts for which we had two annotators to measure the agreement. 
We computed  Krippendorff’s alpha \cite{Krippendorff2011ComputingKA} to measure inter-annotator agreement and found a moderate level of agreement with an alpha coefficient of 0.54. 
We further utilize ChatGPT for evaluating the same 150 samples, as LLMs have demonstrated their effectiveness as evaluators for text generation tasks \cite{luo2023chatgpt, liu2023geval, gao2023humanlike, fu2023gptscore}. We define the informativeness criteria and rating scheme to ChatGPT and then employ ChatGPT to generate evaluation steps. We then send these evaluation steps along with the data table of the chart and the summary to ChatGPT to obtain ratings (see  \Cref{app:human-chatgpt-eval} for details). 


\Cref{tab:informativeness} shows the result of human evaluation on chart summarization based on informativeness criteria. We notice that annotators preferred ZeroShot version of our model which generates summaries that are more similar to those generated by GPT, rather than gold summaries. The finetuned version of \model\ was also rated higher
compared to SoTA MatCha \cite{liu2022matcha}. The finetuned UniChart model also produces fewer factual errors compared to Matcha and the ZeroShot version (\Cref{app:human-chatgpt-eval} and \Cref{tab:human_eval}). We observe that the ratings provided by ChatGPT are roughly consistent with the human annotators' scores in terms of informativeness criteria. Moreover, we conducted a statistical test (p-value) for ratings from humans and ChatGPT, with the null hypothesis that the ratings are two independent samples. The p-values in each row in Table 3 demonstrate that it is very infrequent that two rating samples are independent based on the observed ratings. Also in terms of different semantic contents, the ZeroShot model tends to contain more sentences with high-level visual patterns and trends.
A previous study finds that such high-level insights lead to more reader takeaways compared to the text describing low-level visual encodings like axes and colors~\cite{stokes2022striking}. Overall, the results above suggest that UniChart model's summaries are more informative with high-level insights and factually accurate than the SoTA (MatCha).


\vspace{-1mm}
\subsection{Time and Memory Efficiency} 
\model\ exhibits significant time efficiency compared to MatCha, as shown in \Cref{fig:inference_time}. The gap in speed is more evident on tasks that require the generation of long output sequences (e.g., Chart-to-Text). This difference in speed can be attributed to MatCha's use of a long input sequence (4K) with a quadratic increase in complexity while \model's\ vision encoder relies on sliding windows with a local attention mechanism that scales linearly with the input image size. Moreover, \model\ boasts a smaller parameter count (201M) compared to MatCha (282M), further contributing to its efficiency. As a result, \model\ is highly suitable for real-world applications that prioritize fast inference speeds. More details are provided in \Cref{app:efficiency}. 

\vspace{-1mm}
\subsection{Error Analysis and Challenges}
We conducted a manual analysis of our model's outputs to identify key challenges faced by existing models.

\noindent \textbf{$\bullet$ {Densely populated charts:}} Our model struggles with extracting insights from chart images that contain numerous data elements densely packed in a limited area.  This is evident in Figure \Cref{fig:error-analysis} (Q3) where our model generates a hallucinated summary due to the complexity of the chart. Increasing model parameters and input image resolution could potentially improve performance in these cases.


\noindent \textbf{$\bullet$ {Numerical reasoning:}} Despite efforts to incorporate mathematical skills, our model still encounters difficulties with complex arithmetic calculations (Q2 in \Cref{fig:error-analysis}).   
Addressing this challenge involves decoupling arithmetic calculations and reasoning steps by employing external program executors that perform the calculations using the equations generated by our model \cite{gao2022pal}. 


\noindent \textbf{$\bullet$ {Factual correctness in generated summaries:}} Factual correctness still poses a challenge for autoregressive language models \cite{lin-etal-2022-truthfulqa,ChatGPT,zhao2023verify}. Although our finetuned UniChart model produced fewer factual errors compared to MatCha (see \Cref{tab:human_eval}), it still generates some  incorrect statements (see Q4 in  \Cref{fig:error-analysis}). This issue can be attributed to factual errors in the pretraining captions generated by ChatGPT.










==> Instruc_Human_eval.tex <==

 
 
 
  
  


 

 
                                             

 


==> Novel_task_samples.tex <==
\begin{table}[t]
 \setlength\extrarowheight{1pt}
 \centering

 
 
 \scalebox{0.74s}{\begin{tabular}{l|c}
  
  \toprule
  
  \multirow{1}{*}{\textbf{Task Group}} & \multirow{1}{*}{\textbf{\#Examples}} \\
\midrule
Pattern and Outlier Detection & 16,977 \\
  Statistical Analysis & 9,148 \\
  Extremum Identification & 6,545\\
  Item Correlations & 6,142 \\
  General Comparison & 4,709\\
  Relative Change Calculation & 4,108\\
  Time Series and Future Value Prediction & 1,944 \\
  Data Point Identification & 1,670\\
  Performance and Result Analysis & 1,396\\
  Data Categorization & 533\\
  Distribution analysis & 280\\
  \bottomrule
  

  
 
 \end{tabular}}
 \caption{\small {The number of generated examples for various groups of new tasks created by GPT-4.
 }
 \vspace{-3mm}
 }
 \label{tab:NovelCounts}
\end{table}




==> Task_chart_count.tex <==
\begin{table*}[t]
 \setlength\extrarowheight{1pt}
 \centering
 
 
 
 \scalebox{0.67}{\begin{tabular}{lcccccc|c}
  
  \toprule
  
  \multirow{1}{*}{Dataset
  } & \multirow{1}{*}{CoT Reasoning} & \multicolumn{1}{c}{Chart Summarization} & 
   \multicolumn{1}{c}{Fact Checking} & \multicolumn{1}{c}{Open-ended QA} &
   \multicolumn{1}{c}{Coding Abilities}& \multicolumn{1}{c}{Novel Tasks} 
 \multicolumn{1}{c}{ Distinct Charts}\\%{Model generated} \\
                                             
  
  \midrule

  Statista   & 736 & 4,159 & 2,047 
  &1,485  & 400 & - &  9,992\\ 

  PlotQA   & 703 & 3977 & 1002 
  & 3966 &  400 & - &  8,199\\

  OECD/OWID   &722 & 3999   
  & 2016 & 3961  & 500 & -&  10,949\\

  WebCrawled   & 2,433 & 41,741 & 2,500 
  & 2,448  & 2,390 & 2,606 &  41,742\\
  \midrule
  Total  & 4,594 & 53,876 & 7,565 & 11,860  & 3,690 & 2,606 & 70,882
  \\ \bottomrule
  
 
 \end{tabular}}
 \vspace{-3mm}
 \caption{\small {breakdown of Distinct charts appearing on different tasks. Some of them appear in more than one task, counting in the total.\mehrad{Table Added. Do we want to marge with table 2?}
 }
 \vspace{-3mm}
 }
 \label{tab:chart_count}
\end{table*}



